Model soups need only one ingredient

Fine-tuning large pre-trained models on a target distribution often improves in-distribution (ID) accuracy, but at the cost of out-of-distribution (OOD) robustness as representations specialize to the fine-tuning data. Weight-space ensembling methods, such as Model Soups, mitigate this effect by averaging multiple checkpoints, but they are computationally prohibitive, requiring the training and storage of dozens of fine-tuned models. In this paper, we introduce MonoSoup, a simple, data-free, hyperparameter-free, post-hoc method that achieves a strong ID-OOD balance using only a single checkpoint. Our method applies Singular Value Decomposition (SVD) to each layer's update and decomposes it into high-energy directions that capture task-specific adaptation and low-energy directions that introduce noise but may still encode residual signals useful for robustness. MonoSoup then uses entropy-based effective rank to automatically re-weigh these components with layer-wise coefficients that account for the spectral and geometric structure of the model. Experiments on CLIP models fine-tuned on ImageNet and evaluated under natural distribution shifts, as well as on Qwen language models tested on mathematical reasoning and multiple-choice benchmarks, show that this plug-and-play approach is a practical and effective alternative to multi-checkpoint methods, retaining much of their benefits without their computational overhead.

==> tables/_table_clip.tex <==
\setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{0.8\columnwidth}{!}{%
        \begin{tabular}{l|cc|c}
        \toprule
        \textbf{Method}\phantom{aaaaaaaaaaaaaaa} & \phantom{aaa}\textbf{ID}\phantom{aaa} & \phantom{a}\textbf{Avg. OOD}\phantom{a} & \phantom{a}\textbf{\textit{Cost}}\phantom{a} \\
        \midrule
        Initialization & 75.4\% & 46.2\% &  \\
        FT model (\modeloodbest) & 78.11\% & 50.67\% & \\
        FT model (\modeloodworst) & 76.53\% & 36.71\% & \\ 
       FT model (\modelidbest) & 80.38\% & 47.96\% & \\ 
        FT model  (\modelidworst) & 74.99\% & 38.64\% & \\ 
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{Prior \textit{Soups}-Merging Methods}} \citep{wortsman2022model}} \\
        \midrule
        Uniform Model Soup & 79.9\% & 51.4\% & 70 \\
       Greedy Model Soup & \textbf{81.0\%} & 50.7\% & 70 \\
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{ModelStock~(Pairwise Models)}} \citep{jang2024model}} \\
        \midrule
       \modelidbest, \modeloodbest & 79.39\% & 50.53\% & 2 \\
        \modelidbest, \modeloodworst & 78.43\% & 49.39\% & 2 \\
        \modelidbest, \modelidworst & 78.32\% & 50.63\% & 2 \\
        \modeloodbest, \modeloodworst & 76.76\% & 48.41\% & 2 \\
        \modeloodbest, \modelidworst & 77.49\% & 51.02\% & 2 \\
        \modelidworst, \modeloodworst & 78.09\% & 47.81\% & 2 \\
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{\methodname~(Single Models)} (ours)}} \\
        \midrule
       \modeloodbest & 78.29\% & \textbf{51.60\%}  & 1 \\
        \modeloodworst & 78.55\%  & 44.21\%  & 1 \\
        \modelidbest & 80.03\%  & 49.95\%  & 1 \\
        \modelidworst & 77.76\%  & 46.54\%  & 1 \\
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{ERank-MonoSoup (Single Models)} (ours)}} \\
        \midrule
        {\modeloodbest (ERank)} & {78.21\%} & {50.91\%} & {1} \\
        {\modelidbest (ERank)} & 80.34 \% & 	48.94\% & {1} \\
        \modeloodworst (ERank) & 78.03\% & 42.78\% & {1}\\
        \modelidworst (ERank) & 77.38\% & 45.22\% & {1}\\
        \midrule
        \multicolumn{4}{l}{\textit{\textbf{\methodname~(Pairs of models Models)} (ours)}} \\
        \midrule
       \modelidbest, \modeloodbest & 80.10\% & 51.37\% & 2 \\
        \modelidbest, \modeloodworst & 78.87\% & 48.37\% & 2 \\
        \modelidbest, \modelidworst & 79.02\% & 50.12\% & 2 \\
        \modeloodbest, \modeloodworst & 78.44\% & 49.26\% & 2 \\
        \modeloodbest, \modelidworst & 78.05\% & 50.48\% & 2 \\
        \modelidworst, \modeloodworst & 78.94\% & 47.79\% & 2 \\
        \bottomrule
        \end{tabular}
    }


    

    


==> tables/_table_qwen.tex <==
\setlength{\tabcolsep}{1pt} 
    \renewcommand{\arraystretch}{1.0} 
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|ccccc} 
        \toprule 
        \textbf{Method} & \textbf{GSM8K} & \textbf{GSM${}_{\text{Plus}}$} & \textbf{GSM8K${}_{\text{Platinum}}$} & \textbf{SciQ} & \textbf{MMLU-Pro-Math} \\ 
        \midrule 
        \textsc{Qwen3-0.6B-Base} & 52.6 & 22.5 & 50.1 & 92.6 & 33.7 \\ 
        \midrule 
        \multicolumn{6}{l}{\textit{{Linear Learning Rate Variants} (\texttt{M-1})}} \\ 
        \midrule 
        \texttt{M-1}  & 55.8 & 29.5  & 55.6 & 94.6  & 35.6 \\ 
        \texttt{M-1} + \textsc{LiNeS} & 56.2 & 30.1 & 56.3 & 94.9 & 36.7\\ 
        \texttt{M-1} + \textsc{\methodname} & \textbf{56.7} & \textbf{30.3} & \textbf{56.7}  & \textbf{95.1} & \textbf{37.2} \\ 
        \texttt{M-1} + \textsc{ERank-MonoSoup} & \textbf{56.9} & \textbf{30.2} & \textbf{56.8}  & \textbf{95.3} & \textbf{37.5} \\ 
        \midrule 
        \multicolumn{6}{l}{\textit{\textbf{Cosine Learning Rate Variants} (\texttt{M-2})}} \\ 
        \midrule 
        \texttt{M-2}  & 56.1 & 30.8 & 58.5 & 94.5 & 35.9  \\ 
        \texttt{M-2} + \textsc{LiNeS} & 56.5 & 31.4 & 58.9  & 95.2 & 36.1 \\ 
        \texttt{M-2} + \textsc{\methodname} & \textbf{56.6} & \textbf{31.7} & \textbf{59.3}  & 95.1 & \textbf{36.6}\\
        \texttt{M-2} + \textsc{ERank-MonoSoup} & \textbf{56.8} & \textbf{31.9} & \textbf{59.4}  & \textbf{95.3} & \textbf{36.9}\\
        \midrule 
        \multicolumn{6}{l}{\textit{\textbf{Cosine Learning Rate with Extended Training} (\texttt{M-3})}} \\ 
        \midrule 
        \texttt{M-3} & 55.9 & 30.6  & 57.3 & 93.5 & 34.8 \\ 
        \texttt{M-3} + \textsc{LiNeS} & 56.3 & 30.8 & 58.1 & 93.8 & 35.2  \\ 
        \texttt{M-3} + \textsc{\methodname} & 56.6  & 31.4 & 58.8 & 94.2 & 35.5  \\ 
        \texttt{M-3} + \textsc{ERank-MonoSoup} & \textbf{56.9}  & \textbf{31.7} & \textbf{59.2} & \textbf{94.5} & \textbf{35.8}  \\ 
        \midrule
        \multicolumn{6}{l}{\textit{\textbf{ModelStock Merging Method}}} \\ 
        \midrule
        (\texttt{M-1}, \texttt{M-2}) & 56.6 & 31.5  & 59.0  & 94.9 & 36.8  \\ 
        (\texttt{M-1}, \texttt{M-3}) & 56.4 & 31.3 & 58.7 & 94.8  & 36.4  \\ 
        (\texttt{M-2}, \texttt{M-3}) & 56.5 & 31.6 & 58.9 & 95.2 & 36.7  \\ 
        \bottomrule 
        \end{tabular}
    }

